Connectivity-Aware Pheromone Mobility Model for Autonomous UAV Networks

UAV networks consisting of reduced size, weight, and power (low SWaP) fixed-wing UAVs are used for civilian and military applications such as search and rescue, surveillance, and tracking. To carry out these operations efficiently, there is a need to develop scalable, decentralized autonomous UAV network architectures with high network connectivity. However, the area coverage and the network connectivity requirements exhibit a fundamental trade-off. In this paper, a connectivity-aware pheromone mobility (CAP) model is designed for search and rescue operations, which is capable of maintaining connectivity among UAVs in the network. We use stigmergy-based digital pheromone maps along with distance-based local connectivity information to autonomously coordinate the UAV movements, in order to improve its map coverage efficiency while maintaining high network connectivity.

==> extra.tex <==
\begin{algorithm}
	\caption{Online DQN with experience replay }
	\label{pseudo:dqn-replay}
	\SetAlgorithmName{Pseudocode}{}
	\LinesNumbered 
	\setcounter{AlgoLine}{0}
	\begin{small}
	    Initialize Q-network\;
	    Initialize action-value function $Q$ with random weights $\theta$\;
	    Initialize target action-value function $\hat{Q}$ with weights $\hat{\theta}=\theta$\;
	    Initialize replay memory $D$ of size 10000\;
	    Initialize total episodes N;
	    
		\For{episode = 0 to N}{
			
			\While{t\leq2000s ~$or$~ coverage\geq90\%}{
			    UAVs choose an action $a$ according to the $\epsilon-greedy$ policy based on Q-network\;
			    Execute action $a$, and observe reward $r_t$ and next state $s’_t$\;
			    Store transition $[s,a,r,s’]$ in $D$;\
			    
			    \For{every 30 transitions stored into D}{
			        Sample random minibatch of M transitions $[s_j,a_j,r_j,s’_j]$ from $D$\;

    			 %   Pass $minibatch_i$ through Q-network to get current Q values\;
    			    
    			    \For{every transition j $[s_j,a_j,r_j,s’_j]$ in $minibatch$}{
    			        Calculate target Q values,
    			        $Y_j=r_j+ \gamma max_{a'}Q(s_j',a_j';\theta)$\;
    			    }
    			    Calculate the MSE Loss, $L=\frac{1}{M}\sum_{j=0}^{M-1}(Y_j-Q(s_j,a_j;\theta))^2$\;
    			    Update Q-network weight ($\theta$)  by minimizing the loss function using ADAM\; 
			    }
			    
			    Every C=3000 (or 100 optimization update) steps reset $\hat{Q}=Q$;\
			 }
	    }
    \end{small}
\end{algorithm}



type2:




	\caption{Online DQN with experience replay }
	\label{pseudo:dqn-replay}
	\SetAlgorithmName{Pseudocode}{}
	\LinesNumbered 
	\setcounter{AlgoLine}{0}
	\begin{small}
	    Initialize Q-network\;
	    Initialize action-value function $Q$ with random weights $\theta$\;
	    Initialize target action-value function $\hat{Q}$ with weights $\hat{\theta}=\theta$\;
	    Initialize replay memory $D$ of size 10000\;
	    Initialize total episodes N;
	    
		\For{episode = 0 to N}{
			
			\While{t\leq2000s ~$or$~ coverage\geq90\%}{
			    UAV chooses an action $a$ according to the $\epsilon-greedy$ policy based on Q-network\;
			    Execute action $a$, and observe reward $r_t$ and next state $s’_t$\;
			    Store transition $[s,a,r,s’]$ in $D$;\
			    t=t+1;\
			    
			    \If{$t\mod{30}==0$}{
			        Sample random minibatch of M=512 transitions $[s_j,a_j,r_j,s’_j]$ from $D$\;

    			 %   Pass $minibatch_i$ through Q-network to get current Q values\;
    			    
    			    Calculate target Q values, $y_j=r_j+ \gamma max_{a'}\hat{Q}(s_j',a_j';\theta)$\;
    			    
    			    Calculate the MSE Loss, $L=\frac{1}{M}\sum_{j=0}^{M-1}(y_j-Q(s_j,a_j;\theta))^2$\;
    			    Perform update on Q-network weights ($\theta$) by minimizing the loss function using an adaptive gradient decent(ADAM)\; 
			    }
			    
			    \If{$t\mod{3000}==0$}{Copy Q-network to target network $\hat{Q}=Q$;\
			    }
			 }
	    }
    \end{small}
\end{algorithm}

type3 
\begin{algorithm}
	\SetAlgorithmName{Pseudocode}{}
	\LinesNumbered 
	\setcounter{AlgoLine}{0}
	\begin{small}
	   % Initialize Q-network\;
	    Initialize action-value function $Q$ with random weights $\theta$\;
	    Initialize target action-value function $\hat{Q}$ with weights $\hat{\theta}=\theta$\;
	    Initialize replay memory $D$ of size 10000\;
	    Initialize total episodes $N$\;
	    
		\For{episode = 0 to N}{
			\While{$t\leq2000s ~or~ coverage\geq90\%$}{
			    UAV chooses an action $a$ according to the $\epsilon-greedy$ policy based on Q-network\;
			    Execute action $a$, and observe reward $r_t$ and next state $s’_t$\;
			    Store transition $[s,a,r,s’]$ in $D$\;
			    $t=t+1$\;
			    
			    \If{$t\mod{B}==0$}{%\For{every 30 transitions stored into D}{
			        Sample random minibatch of $M=512$ transitions $[s_j,a_j,r_j,s’_j]$ from $D$\;
    			    
    			    Calculate target Q values, $y_j=r_j+ \gamma max_{a'}\hat{Q}(s_j',a_j';\theta)$\;
    			    
    			    Calculate the MSE Loss, $L=\frac{1}{M}\sum_{j=0}^{M-1}(y_j-Q(s_j,a_j;\theta))^2$\;
    			    Perform update on Q-network weights ($\theta$) by minimizing the loss function using an adaptive gradient decent(ADAM)\; 
			        
			        Every $C$ updates copy Q-network to target network, $\hat{Q}=Q$\;
			    }
			 }
	    }
    \end{small}
	\caption{Online DQN with experience replay }
	\label{pseudo:dqn-replay}
\end{algorithm}
